MDAPT: Multilingual Domain Adaptive Pretraining in a Single Model

Domain adaptive pretraining, i.e. the continued unsupervised pretraining of a language model on domain-specific text, improves the modelling of text for downstream tasks within the domain. Numerous real-world applications are based on domain-specific text, e.g. working with financial or biomedical documents, and these applications often need to support multiple languages. However, large-scale domain-specific multilingual pretraining data for such scenarios can be difficult to obtain, due to regulations, legislation, or simply a lack of language- and domain-specific text. One solution is to train a single multilingual model, taking advantage of the data available in as many languages as possible. In this work, we explore the benefits of domain adaptive pretraining with a focus on adapting to multiple languages within a specific domain. We propose different techniques to compose pretraining corpora that enable a language model to both become domain-specific and multilingual. Evaluation on nine domain-specific datasets-for biomedical named entity recognition and financial sentence classification-covering seven different languages show that a single multilingual domain-specific model can outperform the general multilingual model, and performs close to its monolingual counterpart. This finding holds across two different pretraining methods, adapter-based pretraining and full model pretraining.

==> tables/classification-main-results-archiv.tex <==
\begin{table*}[h!]
    \centering
    \begin{tabular}{r cccc}
    \toprule
    & \bf \GMPCexp-2 & \bf \GMPCexp-9 & \bf \DanFin & \bf \FPBshort \\ 
    & \de & \de & \da & \en \\ 
    \midrule
    & \multicolumn{4}{c}{\textsc{Full model pretraining}} \\
    \midrule
    % \PTmonospecific & - & - & - & 84.7\scriptsize{$\pm$ 1.3} \\
    % \PTmono   & 91.4\scriptsize{$\pm$ 0.3} & 71.5\scriptsize{$\pm$ 0.8} & 65.2\scriptsize{$\pm$ 1.1} & 85.0\scriptsize{$\pm$ 1.0} \\  
    % \PTmulti  & 90.8\scriptsize{$\pm$ 0.4} & 71.1\scriptsize{$\pm$ 0.4} & 62.8\scriptsize{$\pm$ 1.1} & 82.4\scriptsize{$\pm$ 1.0} \\  
    % \adxen    & 91.1\scriptsize{$\pm$ 0.5} & 71.5\scriptsize{$\pm$ 1.0} & 62.7\scriptsize{$\pm$ 1.8} & 83.8\scriptsize{$\pm$ 0.6} \\ 
    % \adxmd    & 91.2\scriptsize{$\pm$ 0.4} & 71.6\scriptsize{$\pm$ 0.5} & 63.6\scriptsize{$\pm$ 1.6} & 83.9\scriptsize{$\pm$ 0.9} \\ 
    % \adxmwiki & 91.3\scriptsize{$\pm$ 0.5} & 71.6\scriptsize{$\pm$ 0.9} & 63.6\scriptsize{$\pm$ 1.6} & 83.6\scriptsize{$\pm$ 0.9} \\ 
    
    De/Da/En-BERT & 91.4 & 71.5 & 65.2 & 85.0 \\ 
\basembert & -0.6 & -0.4 & -2.4 & -2.6 \\ 
\basembert + \adxen & -0.3 & 0 & -2.5 & -1.2 \\ 
\basembert + \adxmd & -0.2 & +0.1 & -1.6 & -1.1 \\ 
\basembert + \adxmwiki & -0.1 & +0.1 & -1.6 & -1.4 \\ 
    
    \midrule
& \multicolumn{4}{c}{\textsc{Adapter-based pretraining}} \\
\midrule
De/Da/En-BERT & 90.5 & 69.1 & 66.0 & 85.3 \\ 
\basembert & -0.0 & 0.8 & -3.1 & -3.1 \\ 
\basembert + \adxen & 0.7 & 1.5 & -4.9 & -3.5 \\ 
\basembert + \adxmd & 0.9 & 3.8 & -1.7 & -2.6 \\ 
\basembert + \adxmwiki & 0.6 & 2.6 & -1.9 & -3.2 \\ 
\bottomrule
    \end{tabular}
    \caption{Evaluation results on classification tasks. We report performance differences compared to the monolingual base-line in terms of accuracy. The reported numbers are averages over 5 runs.}
    \label{table-main-results-financial}
\end{table*}

==> tables/ner-main-results-archiv.tex <==
\iffalse
\begin{table*}[h!]
    \centering
    \begin{tabular}{r | r | ccccc}
    \toprule
    \multirow{2}{*}{\bf Approach} & \multirow{2}{*}{\bf Data} & \bf \quaero & \bf \bioro & \bf \pharmaconershort & \bf \ncbishort & \bf  \\ 
    & & \small Fr & \small Ro & \small Es & \small En & \small Pt \\ 
    \midrule
    \multirow{6}{*}{Full fine-tuning} 
     & \PTmonospecific & - & - & - & 87.9\scriptsize{$\pm$ 0.2}&\\
    & \PTmono & 61.87\scriptsize{$\pm$ 0.3}& 75.1\scriptsize{$\pm$ 0.3}&88.0\scriptsize{$\pm$ 0.7} &85.1\scriptsize{$\pm$0.6 }&  \\  
    & \PTmulti & 58.7\scriptsize{$\pm$ 0.3}& 74.6\scriptsize{$\pm$ 0.6}&87.9\scriptsize{$\pm$ 0.6} &85.8\scriptsize{$\pm$ 0.7} & \\
   
    & \adxen & 59.4\scriptsize{$\pm$ 0.5} &73.8\scriptsize{$\pm$ 1.0} &89.0\scriptsize{$\pm$ 0.6} & 86.8\scriptsize{$\pm$ 1.0}&\\  
    & \adxmd & 60.7\scriptsize{$\pm$ 0.3}&74.3\scriptsize{$\pm$ 0.4} & 88.4\scriptsize{$\pm$ 0.6} & 87.4\scriptsize{$\pm$ 0.5}&\\  
    & \adxmwiki & 60.4\scriptsize{$\pm$ 0.4}&74.4\scriptsize{$\pm$ 0.9}  & 88.7\scriptsize{$\pm$ 0.8}  & 86.6\scriptsize{$\pm$ 0.6}&\\  
    \midrule
\multirow{5}{*}{Adapter-based} & \PTmono & 0.0 \scriptsize{$\pm$ 0.0} & 73.2 \scriptsize{$\pm$ 0.5} & 86.6 \scriptsize{$\pm$ 0.3} & 82.6 \scriptsize{$\pm$ 0.8} \\ 
& \PTmulti & 54.1\scriptsize{$\pm$ 0.5} & 68.7\scriptsize{$\pm$ 0.5} & 86.3\scriptsize{$\pm$ 0.5} & 82.8\scriptsize{$\pm$ 0.3} \\  
& \adxen & 55.8\scriptsize{$\pm$ 0.9} & 71.5\scriptsize{$\pm$ 0.6} & 88.2\scriptsize{$\pm$ 0.3} & 84.0\scriptsize{$\pm$ 0.6} \\  
& \adxmd & 57.3\scriptsize{$\pm$ 0.3} & 71.3\scriptsize{$\pm$ 0.3} & 88.4\scriptsize{$\pm$ 0.3} & 84.0\scriptsize{$\pm$ 0.2} \\  
& \adxmwiki & 56.9\scriptsize{$\pm$ 0.3} & 70.6\scriptsize{$\pm$ 0.4} & 87.4\scriptsize{$\pm$ 0.7} & 83.9\scriptsize{$\pm$ 0.3} \\    
    \bottomrule
    \end{tabular}
    \caption{Evaluation results on NER, in terms of span-level F1 score. Averaged over 5 runs, standard deviation indicated in small}
    \label{table-main-results}
\end{table*}
\fi


\begin{table*}[h!]
    \centering
    \begin{tabular}{l l ccccc}
    \toprule
    && \bf \quaero & \bf \bioro & \bf \pharmaconershort & \bf \ncbishort & \bf \ptner  \\ 
    && \small Fr & \small Ro & \small Es & \small En & \small Pt \\ 
    \midrule
    && \multicolumn{5}{c}{\textsc{Full model pretraining}} \\
    \midrule
 \multirow{2}{*}{PT}   &Fr/Ro/Es/En/Pt-BERT & 61.9& 75.5&88.0 &85.1& 72.3 \\  
    
    %\basembert & 58.7\scriptsize{$\pm$ 0.3}& 74.6\scriptsize{$\pm$ 0.6}&87.9\scriptsize{$\pm$ 0.6} &85.8\scriptsize{$\pm$ 0.7} & \\
    
   &\basembert & -3.8& -1.6&-0.1 &+0.7 & +0.2\\
   
    %\basembert + \adxen & 59.4\scriptsize{$\pm$ 0.5} &73.8\scriptsize{$\pm$ 1.0} &89.0\scriptsize{$\pm$ 0.6} & 86.8\scriptsize{$\pm$ 1.0}&\\  
    
\multirow{3}{*}{\multispecificmodel}    &\basembert + \adxen & -2.9 &-1.6 &+1.0 & +1.7&\\  

    
    %\basembert + \adxmd & 60.7\scriptsize{$\pm$ 0.3}&74.3\scriptsize{$\pm$ 0.4} & 88.4\scriptsize{$\pm$ 0.6} & 87.4\scriptsize{$\pm$ 0.5}&\\  
    
    &\basembert + \adxmd & -2.2&-0.9 & +0.4 & +2.3&\\  
    
    
    %\basembert + \adxmwiki & 60.4\scriptsize{$\pm$ 0.4}&74.4\scriptsize{$\pm$ 0.9}  & 88.7\scriptsize{$\pm$ 0.8}  & 86.6\scriptsize{$\pm$ 0.6}&\\  
    
    &\basembert + \adxmwiki & -1.9&-1.4  & +0.7  & +1.5&\\  
    
    
    \midrule
&& \multicolumn{5}{c}{\textsc{Adapter-based pretraining}} \\
\midrule
&Fr/Ro/Es/En/Pt-BERT & 0.0 & 73.2 & 86.6 & 82.6 & 63.5 \\ 
&\basembert & 54.1 & -4.5 & -0.3 & 0.1 & 0.0 \\ 
&\basembert + \adxen & 55.7 & -2.0 & 1.5 & 1.4 & 3.2 \\ 
&\basembert + \adxmd & 57.3 & -1.9 & 1.9 & 1.4 & 2.8 \\ 
&\basembert + \adxmwiki & 57.2 & -2.6 & 1.0 & 1.8 & 2.3 \\ 
\bottomrule
    \end{tabular}
    \caption{Evaluation results on NER tasks. We report performance differences compared to the monolingual baseline in terms of span-level F1 score. The reported numbers are averages over 5 runs.}
    \label{table-main-results}
\end{table*}


